Think More or Look Again? Training-Free Test-Time Scaling for Multi-Image Medical Reasoning

Medical image interpretation often requires integrating complementary evidence distributed across multiple imaging sequences. Although test-time scaling may improve model performance by allocating additional inference computation, extending textual reasoning alone can reduce visual grounding. We study staged visual inference, a training-free strategy in which a vision-language model first interprets one imaging sequence and subsequently receives complementary images while preserving its inference prefix. Experiments with Qwen3.5-9B and InternVL3.5-8B on a balanced cohort of 90 patients with brain MRI examinations show that the timing and direction of evidence presentation materially affect diagnostic performance. Presenting T2 before T1CE improves balanced accuracy over the corresponding joint-input baseline by 16.7 and 11.1 percentage points for Qwen3.5-9B and InternVL3.5-8B, respectively. These gains are not reproduced by text-only continuation, which consistently increases prediction instability and reduces accuracy. Built-in thinking also incurs substantially greater token and latency costs and can degrade staged inference. Evaluation on prostate and liver MRI demonstrates that the benefits transfer selectively across datasets and models. Overall, staged visual presentation can support diagnostic revision without retraining or architectural modification, but its effectiveness depends on sequence order, model behavior, and the clinical task.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
